A Natural-language-based Visual Query Approach of Uncertain Human Trajectories

Visual querying is essential for interactively exploring massive trajectory data. However, the data uncertainty imposes profound challenges to fulfill advanced analytics requirements. On the one hand, many underlying data does not contain accurate geographic coordinates, e.g., positions of a mobile phone only refer to the regions (i.e., mobile cell stations) in which it resides, instead of accurate GPS coordinates. On the other hand, domain experts and general users prefer a natural way, such as using a natural language sentence, to access and analyze massive movement data. In this paper, we propose a visual analytics approach that can extract spatial-temporal constraints from a textual sentence and support an effective query method over uncertain mobile trajectory data. It is built up on encoding massive, spatially uncertain trajectories by the semantic information of the POIs and regions covered by them, and then storing the trajectory documents in text database with an effective indexing scheme. The visual interface facilitates query condition specification, situation-aware visualization, and semantic exploration of large trajectory data. Usage scenarios on real-world human mobility datasets demonstrate the effectiveness of our approach.

==> honeycomb.tex <==

%Our visual analytics approach consists of two stages (Figure~\ref{fig:pipeline}) : The \textbf{Representation stage} restructured and textualized the massive uncertain trajectories into a semantics-aware representation. The \textbf{Visual Analysis stage} visualized and explored trajectories over map and its semantic meaning.


%%%%%%%%%%%%%%%%%honeycomb%%%%%%%%%%%%%%%%%%%%%%%
%The hierarchy of our new presentation contains three levels, which is constructed recursively from a set of trajectories together with their vectorized representations (described in Section 4.2).
%\textbf{The first level} is constructed by performing a \textit{k}-Means algorithm~\cite{Hartigan1979A} to the input set of trajectories. Each trajectory is encoded with the vectorized representation described above, and the cosine distance between a pair of vectors is used to evaluate their similarity.
%\textbf{The third level} provides a data summarization with respect to the spatial distribution. Two trajectories belong to a cluster if and only if they commonly pass at least one region (covered by a mobile cell station).
%To support level-of-details exploration,  we represent each cluster of each level with its centroid element that is computed by the \textit{k}-Means algorithm. The proposed hierarchy provides a comprehensive view to explore the semantic and spatial distribution of trajectories. Section 6 presents the visualization, exploration and analysis of massive trajectories based on this representation.
%Illustrating the hierarchal structure of trajectories can be fulfilled with conventional tree visualization techniques, like treemap, node-link views or flow map. We design a new visual encoding, called HoneyComb, to account for two considerations. First, the visualization should be spatially compact while preserving the coherence in both the vector space (semantics) and the geographical space (regions). In other words, two trajectories that are near either in the vector space or in the geographical space should be placed near in the visualization. Second, achieving satisfying aesthetics of the visualization  requires an appropriate  aspect ratio while preserving the hierarchy among trajectories.
%Our solution is inspired by the honeycomb, which consists of a set of seamlessly neighbored hexagons, and delivers a compact placement of a group of cells.  While it is easy to construct a honeycomb chart with hexagons, reformulating the semantics-aware representation of the trajectory set (denoted as the trajectory tree) into a set of hexagons and meanwhile satisfying two requirements, is challenging. This requires generating a hierarchical honeycomb structure that hosts three levels of the trajectory tree. The nodes in every level of the representation are then recursively mapped into the corresponding nodes in the honeycomb structure.

%The generated honeycomb structure inherits the hierarchy from the trajectory tree. Each leaf node is filled with a color that encodes the similarity between the node with the queried POI in the context of the semantics-aware representation of a trajectory.  In particular, the semantics of the queried POI denotes the average values of the representations of all trajectories that pass the POI. In this way, the relevances of all leaf nodes of the trajectory tree to the queried result are depicted within a colored honeycomb chart, as shown in \ref{Teaser}.
%The mapping process starts by specifying a center of the honeycomb chart, in which the first tree node is placed. The first node denotes the first leaf node by traversing the trajectory tree in the depth-first order. Thereafter, other leaf nodes in the tree are recursively traversed in a depth-first order with a minimum priority queue.  Every selected node is placed along a radially spiral path (\ref{fig:honey} (b)). Specifically, its location is computed by:
%\begin{eqnarray}
%        D = \sqrt{\frac{x}{w}^{2} + \frac{y}{h}^{2}}
%    \label{eqn:trajn}
%\end{eqnarray}
%where $w$ and $h$  denote the width and height of the visualization, respectively.
%When a leaf node is placed, the priority queue pops an empty node that has the minimum priority and its neighbors are inserted into the queue.
%\begin{figure*}[!htbp]
% \centering
% \includegraphics[width=\linewidth]{honey}
% \caption{The layout of the trajectory tree with a honeycomb chart.}
% \label{fig:honey}
%\end{figure*}
%\ref{algorithm:vHomb} summarizes the layout scheme for constructing the honeycomb structure. The entire process starts from a trajectory tree (\ref{fig:honey} (c)), and progressively produces a honeycomb chart (\ref{fig:honey} (d)).
%\begin{algorithm}[tbp]
%\caption{The layout algorithm for the honeycomb structure}
%\label{algorithm:vHomb}
%\LinesNumbered
%\KwIn{Nodes in the first level: $[C_0, C_1, C_2, \ldots]$; Each $C_i$ contains Nodes in the second level: $[G_1, G_2, G_3, \ldots]$; Each $G_i$ contains Leaf nodes in the third level: $[U_1, U_2, U_3, \ldots]$.}
%\KwOut{output result}%Êä³ö
% $q$: Priority Queue. \;
%Find a layout center $O$, and push empty cell of $O$ into $q$ \;
%\For{each nodes $C_i$}{
%   Find a empty cell P nearest to $O$ by q\;
%   Define P as $C_i$'s layout center\;
%    \For{each nodes $G_j$ in $C_i$}{
%        Find a empty cell T nearest to P by q\;
%        Define T as $G_i$'s layout center\;
%        \For{each nodes $U_m$ in $G_i$}{
%            Find a empty cell K nearest to T by q\;
%            Put $U_m$ in K\;
%            Pop K from $q$\;
%            Push empty cell in the 6 nearest neighbors of K\
%            and K' distance to layout center into $q$\;
%        }
%    }
%}
%\end{algorithm}

==> oldversion/a4.Relevance.tex <==
\subsection{Relevance Quantification}\label{sec:interface}
衡量用户的输入和过滤的轨迹之间的相似性

\noindent \textbf{Relevance between input and trajectories}
\zhaosong{[input sentence, mainly focus on : (1) distance in word space, (2) distance between Keywords and POI]}


\noindent \textbf{Relevance between specification and trajectories}
\zhaosong{[specify a trajectory or spaital-temporal Restraint and resort the result list]}


==> oldversion/a4.Representation.tex <==
4.\section{Uncertainty-aware Representation of Trajectories}
\label{sec:UncertainRepresentation}
An uncertain trajectory gives a series of fuzzy locations related to one mobile object instead of accurate longitudes and latitudes. 
%M: An uncertain trajectory is represented by a series of fuzzy locations related to one mobile object instead of its accurate longitudes and latitudes.
For example, on human mobile trajectories, each sampling point only tells us the mobile station that the mobile phone is connected to, as shown in Figure~\ref{fig:region}. It is hard to identify the specific destination because there exists no unique POI we can determine in the region covered by the mobile station.
%M: Take a mobile trajectory as an example, each sampling point only tell the mobile station that the mobile phone is connected to, as shown in Figure~\ref{fig:region} 

However, analyzing the functionality of the regions can help speculating the possible destinations of the trajectories. For example, if a trajectory ends in an area that has entertainment functionality at noon, its destination tends to be a restaurant instead of a hospital.
We propose a semantics-aware representation described below for exploiting the semantics of a region to enrich the uncertainty of trajectories. In this paper, we use human mobile trajectory data to introduce our method. Note that it is easy to extend the representation method to other kinds of uncertain trajectory data.



\begin{figure}[!htbp]
 \centering
 \includegraphics[width=\columnwidth]{siteregion}
 \caption{Illustration of the Voronoi partition and the uncertainty of a trajectory.}
 \label{fig:region}
\end{figure}



\subsection{Region Textualization and Probabilistic Functionality}\label{sec:Textualization}

Functionality representation and analysis of the spatial regions is essential to understand human behaviors. However, the functionalities of spatial regions are difficult to distinguish because of their diversity and complexity growing up with the development of city~\cite{Yuan:2012:Discovering}. We novelly develop a probabilistic representation which can efficiently extract the functionalities of spatial regions based on the related POIs through textualization and topic modeling. 
%Diverse functional regions, such as business districts and residence community, are growing up with the development of city~\cite{Yuan:2012:Discovering}. Analyzing related POIs can reveal the corresponding functionalities of a spatial region. For example, if government buildings and museums are distributed in one district extensively, this region is likely related to public administration and education. Extracting such kind of knowledge offers a new opportunity for exploring and understanding human movement data.

Probabilistic topic models (e.g., pLSA~\cite{Hofmann1999Probabilistic} and LDA~\cite{Blei2003Latent}) have been successfully used to extract hidden themes from a large archive of documents. The observation behind the topic models is that documents exhibit multiple topics, and each word in the document supports some specific topics. The relation between words, topics, and documents can be computed based on the topic models. Fortunately, the topic model is easily scaled to extract hidden functional semantics of a spatial region. By regarding regions as documents and POIs as words, LDA topic model will generate many topics and each spatial region will exhibit several hidden topics which denote their function.

More specifically, given a region $R$, we collect all types of POIs in $R$ and use them as the words in a region document. These types are usually defined for describing the functionality of one POI (e.g., shop, restaurant). For instance, a document for the one in the northwest of Figure~\ref{fig:region} contains five words:  (restaurant, restaurant, restaurant, restaurant, shop). Subsequently, all regions documents are fed into the LDA topic model, resulting in two relation matrices: a word-topic matrix and a topic-document matrix. The word-topic matrix explains the semantics of topics which shows the degree of correlations between a POI type and a topic. The topic-document matrix reveals the relevance of a topic with a region subject to the semantics of regions. Formally, the semantics of a region $R$ is represented as $S_R = (q_0,  q_1,\ldots, q_n)$, where each $q_i$ denotes the proportion of a topic $t_i$ in $R$. In Figure~\ref{fig:region}, the semantics of the northwest partition is represented by its topics and topic-document possibility, namely, `catering' and `entertainment' with the proportions of 80\% and 18\%, respectively.

\subsection{Probabilistic Representation of Trajectory}
\label{sec:ProbabilisticRepresentation}
Once a region's probabilistic functionalities are computed, the uncertainty-aware representation of an uncertain trajectory is achieved by utilizing the fuzzy regions of its sampling locations.

For a trajectory of $(m_0, m_1, \dots, m_n)$, where $m_i$ is a fuzzy location (e.g., a mobile tower station). The uncertainty representation is given by Equation~\ref{equation:RT}.
\begin{equation}\label{equation:RT}
S_{T} =((S_{m_0},t_0),(S_{m_1},t_1),\ldots,(S_{m_n},t_n))
\end{equation}
where $S_{m_i}$ and $t_i$ denotes the extracted semantics of the corresponding region and the corresponding time stamps of $m_i$.

Technically, $S_{m_i}$ should be acquired by defining a region around $m_i$ and then using the region's functional probabilities computed in the above subsection. Given a distribution of mobile stations, we partition the underlying space into such regions by applying the Voronoi-diagrams partitioning~\cite{aurenhammer1991voronoi}. Voronoi-diagrams algorithm yields a set of disjoint Voronoi cells in a city. Each city POI uniquely belongs to a certain partitioned region, and each region contains a cell station and multiple (could be more than one hundred) POIs (Figure~\ref{fig:region}). After textualizing these Voronoi regions and computing the LDA topics, the trained topics-document matrix shows the relevance of the topics to each region. Then, a trajectory consisting of a series fuzzy locations can be encoded as a series of locational semantics as $S_T = (S_{m_0}, S_{m_1}, S_{m_2}, ...)$. Here each $S_{m_0}$ refers to the topic probabilities at one location, such as $S_{m_0}$ = \{(residence community, 0.7), (business area, 0.1), (transportation area, 0.2)\}, \{(educational area, 0.5), (business area, 0.5)\}, \{(tourist area, 0.6), (shopping area, 0.4)\}, where each pair denotes the topic name with its probabilistic relevance to the region, respectively. In this way, we define a probabilistic representation of the uncertain trajectories, which reflects their possible behavior functions along the moving path.

\subsection{Operating Trajectories}\label{sec:CT}
Given the vectorized representation of uncertain trajectories, many operations about trajectories can be executed to perform complicated analytic tasks. Here we list the typical tasks:
\begin{itemize}
    \item \textbf{Comparing Trajectories:} Several existing works focus on the comparison of different trajectories $T_1$ and $T_2$. For example, Lee et al~\cite{lee2007trajectory} proposed a Partition-and-Group framework where MSTP-Similarity~\cite{ying2010mining} takes semantics into account to measure the similarity between two trajectories. In this paper, we use Equation~\ref{equation:R}, which extend the Levenshtein distance algorithm, to quantify the similarity between the semantics of two trajectories. The main idea is to calculate the minimum number of changes (deletions, insertions or movement) required to change one trajectory into the other.
\begin{equation}\label{equation:R}
R = \omega_1\sum_{(i,j)\in S}\delta (T_{1_i},T_{2_j})+\omega_2(\sum_{i\in\bar{S}}\gamma (T_{1_i})+\sum_{j\in \bar{S}}\gamma (T_{2_j}))  
\end{equation}
$S$ represents a set of matching GPS points over trajectory $T_1$ and $T_2$ and $\bar{S}$ contains GPS points over $T_1$ and $T_2$ that are not included in $S$. $\delta(T_{1_i},T_{2_j})$ equals to the distance between vector $T_{1_i}$ and $T_{2_j}$, $\gamma (T_{1_i})$ equals to norm of vector $T_{1_i}$. $\omega_1$ and $\omega_2$ are two adjust parameters. 

To minimize Equation~\ref{equation:R}, we seek to find as many matching points between $T_1$ and $T_2$ as possible, and to ensure that the distance between corresponding vectors of matched points is as small as possible. Thus, we should maximize the size of $S$ and minimize the first part of Equation~\ref{equation:R}, which is equivalent to solve the Ordered minimum weighted match (MWM) problem of the bipartite graph, where each node set represents a trajectory. We generate a complete weighted bipartite graph $G$, which has node set $\left \{ T_{1_1},T_{1_2},T_{1_3},....,T_{1_n} \right \} \times \left \{ T_{2_1},T_{2_2},T_{2_3},....,T_{2_m} \right \}$, where $n$ and $m$ is the length of $T_1$ and $T_2$, $T_{1_i}$ denotes the semantics of i-th GPS point over $T_1$. The edges of $G$ have weights which equal to the distance between vectors of nodes. Then, finding Ordered MWM of the bipartite graph can be easily solved by running KM algorithm~\cite{lin2009matchsim}.
    \item \textbf{Filtering Trajectories:} Filtering the human trajectories based on stopover time or semantic information is easy to achieve. For example, the manager of a supermarket wants to investigate where people go to their supermarket to optimize the shuttle bus schedules. So the manager can filter the trajectories by giving the conditions of starting from residential communities and stay at the market area for at least 2 hours. The semantic filtering can be implemented by applying thresholds over the probabilistic values (such as residential communities probability bigger than 0.7) and the stopover time on a trajectory. Note that the stopover time can be obtained by calculating the time interval between two timestamps. The relevance of queried trajectories and querying conditions is important for visual exploring the queried results.
    \item \textbf{Clustering Trajectories:} Trajectories clustering can be executed by employing clustering algorithm on their vectorized representations. A typical task is to classify trajectories with their home or workplace. Examining the semantics and the stopover time of GPS points can extract the home or workplace of trajectories. For example, the location in a residential community that a trajectory stays all night long for several days can be regarded as home. Then, K-means algorithm can be performed on the extracted semantic vectors of home and workplace to classify trajectories.
\end{itemize}


==> oldversion/a5.document.tex <==
\section{Searching Engine}\label{sec:Indexing}
Managing trajectory data for semantic querying requires an optimized storage and indexing scheme. Challenges lie in that trajectories are massive, semantic and spatiotemporal.
%M: Efficient semantic query processing for trajectory data requires an optimized data storage and indexing, especially for massive trajectory data with textual information. 

\subsection{Documentation}
\label{sec:trajectorydocument}
The procedure to transform a trajectory into a text-compatible formulation is called \textbf{trajectory documentation}. 
%M: The procedure to encode a trajectory with a text-compatible formulation is called \textbf{trajectory documentation}. 
The goal is to enrich trajectory data with its contextual information and build an effective storage strategy. 
%M: remove The goal. 
As shown in Figure~\ref{fig:trajectorydocument}, we encode a trajectory with its corresponding attributes of GPS points staying along this trajectory. The attributes includes trajectory ID, POI name and type in this work.
The associated attributes of a GPS point including:
\begin{itemize}
    \item \textbf{Timestamp:}  Timestamp is considered as temporal information and can be converted to a descriptive term. For example, 00:00 $pm$ is usually transformed as ``noon''.
    \item \textbf{Linked Mobile Station:} Each GPS point of human mobile trajectory gives the linked mobile station with its station ID, latitude, and longitude which can be regarded as spatial information about the trajectory.
    \item \textbf{Covered POIs:} Running Voronoi diagram algorithm on all mobile stations gives several partitioned regions. Each GPS point is given by its linked mobile station which corresponding to a partitioned region and contains a collection of POIs. The names and types of these covered POIs denote the semantic contextual information. 
\end{itemize}

Therefore, the sequence of GPS points for one trajectory are mapped to a composition of words which denotes both spatial-temporal and semantic information of the trajectory.
\begin{figure}[!htbp]
 \centering
 \includegraphics[width=\columnwidth]{trajectorydocument}
 \caption{Illustration of our trajectory documention scheme.}
 \label{fig:trajectorydocument}
\end{figure}


\subsection{Indexing}
We propose a \textbf{temporal-textual-trajectory index} to support efficient semantic query. 
First, the collection of trajectory documents is divided into multiple data partitions based on a time interval, that is, trajectories staying in the same time window are fetched and storied into the same data partition. Then, trajectory documents in the same partition are stored into adjacent disk blocks to save disk I/O. Next, we build an inverted index for trajectory documents in the same data partition. This inverted index consists of a list of unique keywords (e.g., covered POIs names, types). For each keyword, we record the IDs of trajectories whose documents contain the keyword. Finally, we propagate the timestamps used for data partitions to the inverted indices and generate a temporal-textual-trajectory index.

For example, given a semantic query condition, such as ``find human trajectories starting from restaurants and ending at a train station in the morning'', data partitions that meet the temporal constraints ``morning'' are first fetched. Because data partitions are sorted by time, a binary search is used to speedup this searching procedure and this runtime overhead is $O(log\;p)$, where $p$ is the total number of data partitions.
After that, for each qualified data partition, the built inverted index finds trajectories that match the textual inputs ``restaurants'' and ``train station''. The second step involves $O(1)$ runtime cost for each partition given by the first step. Query trajectories that meet spatial-temporal constraints can be filtered out as well by a similar procedure, which uses the ID of mobile stations that satisfy the spatial constraint as the textual input. Our experiment results show the index can accelerate semantic query over massive trajectories, and achieve less latency for real-time exploration and visualization.

==> oldversion/a6.interface.tex <==


\section{Visual Analysis}\label{sec:interface}
%In this paper,  we work on the following visual analytic tasks:
%\begin{itemize}
%    \item \textbf{T1 Semantic query}: The users with no prior knowledge want to perform a query with semantics-aware text input which contains a sequence of daily used words (e.g., names or types of POIs) and other constraints, like specific spatial region selected from map or time intervals defined by a time-picker selection. 
%    \item \textbf{T2 Detailed inspection of trajectory semantics}: The semantics of one or multiple trajectories should be expressively illustrated for detailed inspection, pairwise comparison or comparative analysis.
%    \item \textbf{T3 Presenting large-scale trajectories}: If there are a large amount of queried trajectories, they should be presented and explored with a level-of-details fashion. A compact yet efficient visual layout of multi-level trajectories is needed.
    %The queried trajectories could still have a large size, and thereby iterative filtering operations are needed.
%    \item \textbf{T4 Uncertainty exploration}:  
%\end{itemize}
%Our visual interface consists of multiple views including, (a) the query view that supports specifying query conditions, (b) the scene view that allows situation-aware exploration of trajectories on map, (c) the semantic view that enables visual analysis, comparison and inspection of semantic trajectories. The scene view is augmented with a configuration widget, (d)configuration panel (e) to help analyst specify the parameters of rendering trajectories and a time control (f) to specify the time interval.

We proposed a visual analytics environment (Figure~\ref{fig:Interface}) to support semantic querying, comparison and situation-aware analysis of uncertain trajectory data. Our interface includes a querying view that allows for specifying query conditions; a semantics view that visualizes the semantic contextual information about trajectories; and a scene view that displays retrieved trajectories on the map with a configuration panel that enables filtering queried results.

\begin{figure}[tb]
 \centering
 \includegraphics[width=\columnwidth]{specify}
 \caption{Illustration for specifying the query conditions. (a) The POI list (b) The time picker widget}
 \label{fig:specify}
\end{figure}
\subsection{The querying view}
The querying view (Figure~\ref{fig:specify}) enables the analyst to specify text-based query conditions. For example, the analyst input ``querying trajectories pass train station during 2014-1-14 morning'' to perform a query. The specified sentence is divided into a sequence of words which denotes the temporal, spatial, and semantic constraint (e.g., names or types of POIs) separately. Constraints are connected by predefined conjunctions to indicate their relations, such as ``during'' and ``pass''. 
We pre-defined several words and conjunctions to denotes temporal constraints and relations between constants. More supported conjunctions and their descriptions are given in Table~\ref{tab:Condition}.


\begin{figure*}[tb]
 \centering
 \includegraphics[width=\linewidth]{interface}
 \caption{Our visual interface consists of multiple views: (a) the query view (b) the scene view (c) the semantic view (d) the configuration panel (e) configuration widget (f) the statistic view.}
    \label{fig:Interface}
\end{figure*}

\begin{table}[tb]
  \caption{Examples of the dictionary of constraints}\label{tab:Condition}
  \scriptsize%
  \begin{tabu}to\linewidth{X[l] X[2.5l]}
  \toprule
  Query Syntax & Description  \\
  \midrule
  morning   & From 6:00 to 9:00 \\
  \midrule
  noon  & From 11:00 to 14:00 \\
  \midrule
  evening   & From 18:00 to 24:00 \\
  \midrule
  pass A   & Trajectory pass a place A \\
  \midrule
  stay A   & Trajectory stay at a place A \\
  \midrule
  during (T)  & Time constraint, where T is a time period\\
  \midrule
  A after B & Trajectory go to place 'B' after place `A'. \\
  \midrule
  A before B  & Trajectory go to place 'A' before place `B'\\
  \midrule
  A or B  & Trajectory go to either place `A' or `B'\\
  \midrule
  A and B  & Trajectory go to both place `A' and `B' \\
  \bottomrule
  \end{tabu}%
\end{table}




In addition to the text-based input, a list of POIs that match the querying conditions are listed. The analyst is allowed to choose specific POIs that need to be passed by the trajectories. For example, the analyst can choose several POIs by drawing a region on the map, or directly select interested POIs from a POI list.

\subsection{The semantics view}
In the semantics view, whereas previous solutions strive for depicting the spatial-temporal information of trajectories, our approach focuses on the depiction of the semantics hidden in uncertain trajectories for efficient analysis and comparison of queried results. Specifically, we design two visual encodings: one for illustrating the semantics of a trajectory, and the other for visual exploration of a set of trajectories.

\noindent \textbf{Visual encoding of a trajectory}
As shown in Figure~\ref{fig:glyph}, an iconic glyph is designed to illustrate the semantics of a trajectory. We utilize a sequence of glyphs connected with line segments to represent a trajectory. Each glyph shows a GPS point about the functionality of its linked mobile station. The Icon in a glyph encodes the dominant functionality. Other possible functionalities are sequentially listed according to their relevance between the functionality and the linked mobile station (Figure~\ref{fig:glyph}). Note that different color represents different functionalities and the circle around the icon, which refer to 24 hours in a day, encodes the stopover time of the GPS point. For example, the left glyph in Figure~\ref{fig:glyph} represent the person stay in a place that may be a tourist area from ``0:00 a.m.'' to ``3:00 p.m.''. The other functionalities of this place are `catering' and `entertainment' with relevance 15\% and 10\%.
\begin{figure}[tb]
 \centering
 \includegraphics[width=\columnwidth]{glyph}
 \caption{Visual encoding for visualizing the semantics of a trajectory.}
 \label{fig:glyph}
\end{figure}

Due to a large number of GPS points over a trajectory and the limitations of the screen, we only encode the GPS points that meet the querying conditions with glyphs at the beginning and merged others into a small folded circle with a number indicates the number of GPS points to get a concise interface.


\noindent \textbf{Visual encoding of a trajectory set}
To support aggregation and summarization for exploring trajectories, we exploit the semantic coherence among trajectories and design a circular glyph for visualizing a set of trajectories with similar semantics as shown in Figure~\ref{fig:setglyph}.
For a trajectory set $S$, we refer the vector which is the centroid of all vectorized representations of trajectories in $S$ as ``central vector''. Composing both the ``central vector'' which summarize the semantics of $S$ and the temporal information of $S$, we adopt a radial layout which arranges a sequence of icon sets and a clockwise statistic graph from inside to outside to visualize $S$. Specifically, the ``central vector'' can be expressed by a sequence of Points with their corresponding functionalities. We encode each point with an icon set where the icons denote the functionalities, and the size of icons denote the relevance between the functionalities and the point. 
For example, the left icon set in Figure~\ref{fig:setglyph} means that the first point of the ``central vector'' has dominant functionality ``entertainment'' and other two relevant functionalities. A statistic graph shows the temporal information of all GPS points. We choose 15-minutes as the time interval of a time frame since Zeng et al.~\cite{Zeng:2017:Visualizing} find that if the temporal interval is less than 15 minutes, the movement regularity will decrease.
In addition, the grayscale of the hexagon represents the relevance between trajectories and querying constraints. The size of hexagonal glyph encodes the number of trajectories in $S$. 
\begin{figure}[tb]
 \centering
 \includegraphics[width=\columnwidth]{combineglyph}
 \caption{Glyph for visualizing the semantics of a set of trajectories.}
 \label{fig:setglyph}
\end{figure}


By clicking and hovering the hexagonal glyph, a statistic graph (Figure~\ref{fig:Statistic}) is shown to help analysts investigate trajectories with their temporal coherence. We combine a matrix graph with a bar chart to organize trajectories. Each row represents a set of trajectories whose timestamps of GPS points that meet the querying conditions are within the same time interval. The red elements denote ``matching points''(GPS points that meet the querying conditions). The other elements encode the number of GPS points with color. The bar chart shows the number of trajectories in a trajectory set. For example, ``Trajectory set 1'' in Figure~\ref{fig:Statistic} represents trajectories whose timestamps of the ``matching point'' are in ``00:00 a.m.'' to ``02:00 a.m.''. Besides, trajectories in ``Trajectory set 1'' are active in the night which can be observed by the time matrix.
\begin{figure}[tb]
 \centering
 \includegraphics[width=\columnwidth]{individual}
 \caption{Statistic graph for investigating the temporal coherence of trajectories.}
 \label{fig:Statistic}
\end{figure}

\noindent \textbf{Configuration panel}
Querying semantic trajectories may lead to a large number of results. To further filter out and Sort trajectories by its relevance to the query conditions, we propose the configuration panel which provides a set of filtering options. Each spatial or semantic constraint (e.g., stay at a region $R$ or ``stay at downtown area'') holds a minimum stopover time option to filters out trajectories whose staying durations of the corresponding GPS point are smaller than a given threshold. Also, each semantic querying condition has a widget which allowed the analyst specify the ideal functionalities' distribution of the matching GPS point. Once the distribution is specified, query results can be sorted according to the relevance between the functionalities' distribution of matching GPS point and the ideal distribution.
%, which can be calculated by the distance between ``central vector'' and inputted standard vector.
%specifying the particular spatial and temporal ranges. favoring modulating the filtering conditions.

\subsection{The scene view}
The scene view (Figure~\ref{fig:Interface} (b)) encodes the filtered trajectories with polylines in the geographical map. The POIs, which are used as querying constraints, are also displayed with representative icons. We also propose a widget (Figure~\ref{fig:Interface} (e)) to help analyst specify the parameters of rendering trajectories, such as color, weight, and opacity of polylines.

To manage the trajectories shown in the scene view, we build a trajectory list to display all the trajectories shown on the map. The analyst is allowed to add trajectories to the scene view by clicking trajectories on the semantics view. Supported interactions including highlighting trajectory while hovering on the trajectory list, zooming in and out on the map. The scene view also supports comparison of trajectories by assigning different colors to trajectories shown on the map on the configuration widget. 

==> oldversion/a7.casestudy.tex <==

\begin{figure*}[tb]
 \centering
 \includegraphics[width=\linewidth]{case2}
 \caption{Illustration of Case 2. (a) The query condition as ``find trajectory pass train station during 2014-1-14'' (b) The query results shown on the scene view and the semantic view (c) the trajectories that stay in a location which have semantics ``restaurant'' (d) the trajectories that that live near the train station (e) the trajectories that shopping at the area which contains the train station.}
 \label{fig:case2}
\end{figure*}
\section{Case Studies}\label{sec:casestudy}
We implemented our prototype with javascript and the MySQL database. All experiments are performed on a PC with an Intel(R) Core(TM) i5-4590 CPU @ 3.30GHz and 24 GB of memory.

We conducted several case studies and experimental comparisons on a real dataset. The dataset contains the trajectories of 14 million citizens in a city  that were collected between Jan. 10th, 2014 and Jan. 31st, 2014. Its total size is 736 GB bytes. Two main components including,
\begin{itemize}
    \item POIs: There are 862,635 POIs, each of which records its GPS coordinates, name and type.
    \item Mobile phone locations: There are 3 billion records of 7 million anonymized mobile phone users. Each record  contains the anonymized User ID, the cell tower ID and the time stamp. The location accuracy varies from 500 to 5000 meters depending on the coverage of cell towers.
\end{itemize}

\noindent \textbf{Data preprocessing:} Taking human mobile trajectory data, station detail records, and POIs data as input, we apply standard data preprocessing  techniques to clean the raw data like removing noise data and completing missing values. Then, our data processing emphasizes on functionalities extracting of regions centered in mobile stations and data storage.
Following the process of textualization which described in Section~\ref{sec:Textualization}, we convert POIs into \emph{words} and then regions are transformed into \emph{documents}. An LDA topic model is applied to characterize the semantic topic of these spatial regions. In practice, we empirically set the semantic topic number to be 13 after several tests. For the sake of clarification, each topic is assigned with a specific name and icon corresponding to a type of functionality area as shown in Figure~\ref{fig:widget}.
To build the temporal-textual-trajectory index, we choose 10 minutes as the window size and select keywords of inverted index including POIs name, POIs type, linked mobile station ID, latitude, longitude and trajectory ID. Fast temporal-spatial query and semantic query can be supported by the built temporal-textual-trajectory index.
The querying results are first transformed into the vectorized representations as described in Section~\ref{sec:ProbabilisticRepresentation}.

\subsection{Case1: Studying the traveling into the hospital}
Our first case is to analyze the medical-related trajectories in the city. The user first defines the query condition as "Query trajectories that pass through the hospital" (Figure~\ref{fig:teaser} (a)). Our system returns a significant amount of trajectory data. We found that there are several hospitals in the central area of the city. The trajectories passing through the area are illustrated in the Figure~\ref{fig:teaser} (b). In the statistics view, We found that some people arrived at the hospital very early. By analyzing their trajectories through the trajectory list and the scene view, we found that they came to the hospital from the rented houses near the area (Figure~\ref{fig:teaser} (c)). The domain exports explain that due to the limited number of medical resources, many people have to arrive early to cure their disease. Another reason is that if the citizens near the hospital have sudden illnesses, they prefer to go to the nearest hospital.

Then, we found another set of trajectories, and they came from the place far away from the city (Figure~\ref{fig:teaser} (d)). To further understand the trajectories, the user defined the query conditions as “query the trajectory from the train station to the hospital during the day,” and then increase the partition of the medical functionality in the area. As shown in (Figure~\ref{fig:teaser} (e)), through the semantic view, we found that there are lots of trajectories come from different locations to the downtown area, the most relevant trajectories are from other hospitals to the hospital, which meaning that these people might be transferred to another hospital. Analyzing their trajectories by looking at the scene view and the trajectory list ((Figure~\ref{fig:teaser} (f))), we found that some of them were moved from hospitals in the Affiliated City into the downtown area. Besides, most of the transfer cases were at noon and afternoon.


Through the visual analysis, we have some interesting finding: (1) People prefer to go to their nearby hospital. (2) There are many people transferred from the Affiliated hospital to the hospital in downtown. There are also several people transferred from the hospital in downtown to the Affiliated hospital. (3) There are many rental houses near the hospital that patients live.
By case1, we demonstrate the ability of our system on querying across the semantic input and the effectiveness to summarize the semantics of large trajectory data.


\subsection{Case 2: Studying the travelling into the train station}
In this case, we illustrate how the proposed approach helps query and analyze trajectories that pass a given location.

First, the analyst performs a query with ``\emph{passing train station during [morning Jan. 14 2014]}'' as the query condition (\ref{fig:case2} (a)). Retrieved trajectories are presented with the semantic view (\ref{fig:case2} (b)). We classify the trajectories into several groups and the group in dark color indicates that the semantics of trajectories is close to the query condition. This guides the analyst to focus on the most relevant trajectories.

After studying the cluster in the scene view and the semantic view, the analyst finds that trajectories are mainly distributed in three areas: the train station, main roads of city and railways. It indicates that most people come to the train station for traveling. Subsequently, the major semantic topic of trajectories is identified as `restaurant' (\ref{fig:case2} (c)) because there are many restaurants around the train station while the other group of trajectories leave city by train (\ref{fig:case2} (d)).



The analyst studies another cluster, in which trajectories show that persons come to the area of the train station but do not move to other cities. The analyst investigates the semantics of trajectories and finds that the topics include service and shopping. This implies that there is a shopping center around the train station (\ref{fig:case2} (e)).

Through the visual analysis, we have following observations: (1) Riding train is the major way for citizens to head to other cities. (2) The dinning service is popular around the train station. (3) The traffic to the train station is not satisyfing. (4) There is a business district near the train station, which has a large traffic flow. These observations are useful in selecting business sites and planning public transportation.


\begin{figure*}[tb]
 \centering
 \includegraphics[width=\linewidth]{case3}
 \caption{Illustration of Case 3. (a) The query condition as ``find trajectory pass college during 2014-1-14'' (b) The query results shown on the scene view and the semantic view (c) The trajectories that go to downtown for shopping (e) The trajectories that go to downtown area in a ``Hospital'' (f) The trajectories that leave the city. (g) The trajectories that live in the college.}
 \label{fig:case3}
\end{figure*}

\subsection{Case 3: Analyzing the daily life in a college}
The analyst specifies ``pass college during [Jan. 10 2014]" and performs the query (\ref{fig:case3} (a)). The results shown on the scene view and the semantic views (\ref{fig:case3} (b)), and it is observed that POIs of qualified trajectories are distributed in an area which is far away from the downtown.
The analyst finds that this is a new campus of a local university. Subsequently, the analyst conducts the analysis in this region (\ref{fig:case3} (d)).
Given that most trajectories distribute between the campus and the downtown, the analyst inferences that the members of the campus visit the downtown frequently (\ref{fig:case3}(c)).

Next, the analyst studies the trajectories visit downtown area and finds that the major topic is ``Hospital" which indicate the students prefer to visit hospital in the downtown area instead of in the campus (\ref{fig:case3} (e)).

The analyst also studies trajectories whose semantics include  ``education". The queried trajectories mainly locate in the campus. This implies that there are many facilities on education around the campus (\ref{fig:case3} (g)).

Finally, the analyst identifies a trajectory cluster that contains the topic ``downtown". By further specifying  ``pass college and pass train station during [Jan. 10 2014]" and performing querying, it is found that these trajectories finally end in the campus and leave the city(\ref{fig:case3} (f)). 

